Active Automata Learning with Adaptive Distinguishing Sequences

This document investigates the integration of adaptive distinguishing sequences into the process of active automata learning (AAL). A novel AAL algorithm "ADT" (adaptive discrimination tree) is developed and presented. Since the submission of the original thesis, the presented algorithm has been integrated into LearnLib - an open-source library for active automata learning - and has been successfully used in related fields of research.

==> alg/adt_refine2.tex <==
\begin{algorithmic}[1]
	\Function{refineHypothesisInternal}{$ce = \langle in, out \rangle$}
	\If{$\lambda(in) = out$}
	\State \Return{false}
	\EndIf
	\Let{$\langle u, a, v \rangle$}{\Call{decomposeCounterExample}{$in$}}
	\Let{$n$}{$\vert S \vert$} \Comment{The new state}
	\Let{$S$}{$S \cup \{n\}$}
	\Let{$accessSequences[n]$}{$accessSequences[\delta(u)] \cdot a$}
	\Let{$\delta(\delta(u), a)$}{$n$} \Comment{MST transition}
	\State \Call{updateADT}{$adt, \delta(ua), n, v$} 
	\Let{openTransitions}{$\{\langle n, i, \cdot, \cdot\rangle \vert i \in I\} \cup \{\langle s, i, \cdot, \cdot\rangle \vert \delta(s, i) = \delta(ua), s \in S, i \in I\}$}
	\State \Call{closeTransitions}{}
	\State \Return{true}
	\EndFunction
\end{algorithmic}


==> figures/dt_3.tex <==

\begin{framedFigure}
	\captionabove{Discrimination Trees and deduced observation table (2)}
	\label{fig:dt_2asdasd}
	\begin{minipage}[]{0.49\textwidth}
		\centering
		\begin{tabular}{r||cc}
			& $water$ & $water \cdot button$\\ \hline \hline
			$\varepsilon$ & \coffeeok & \coffeeerror \\
			$button$ & \coffeeerror & \\ 
			$pod$ & \coffeeok & \coffeecup \\ \hline
			$water$ & \coffeeok & \coffeeerror \\
			$clean$ & \coffeeok & \coffeeerror \\
			$button \cdot water$ & \coffeeerror & \\
			$button \cdot pod$ & \coffeeerror & \\
			$button \cdot button$ & \coffeeerror & \\
			$button \cdot clean$ & \coffeeerror & \\
			$pod \cdot water$ & \coffeeok & \coffeecup \\
			... & ... & ...
		\end{tabular}
	\end{minipage}
	\begin{minipage}[]{0.49\textwidth}
		\centering
		\begin{tikzpicture}[->,thick,>=stealth']
			\node[state,ellipse] (w) at(0,0) {$water$};
			\node[state,ellipse] (wb) at(-2,-2) {$water \cdot button$};
			\node[draw,rectangle] (b) at(2,-2) {$q_b$};
			\node[draw,rectangle] (e) at(-3,-4) {$q_{\varepsilon}$};
			\node[draw,rectangle] (p) at(-1,-4) {$q_{p}$};

			\draw (w) edge node[anchor=south east] {\coffeeok} (wb);
			\draw (w) edge node[anchor=south west] {\coffeeerror} (b);
			\draw (wb) edge node[anchor=south east] {\coffeeerror} (e);
			\draw (wb) edge node[anchor=south west] {\coffeecup} (p);

		\end{tikzpicture}
	\end{minipage}
\end{framedFigure}





==> sections/titelseite.tex <==
\begin{titlepage}
\definecolor{TUGreen}{rgb}{0.517,0.721,0.094}
\vspace*{-2cm}
\newlength{\links}
\setlength{\links}{-1.5cm}
\sffamily
\hspace*{\links}
\begin{minipage}{12.5cm}
\includegraphics[width=8cm]{images/tud_logo.pdf}
%\hspace*{-0.25cm} \textbf{TECHNISCHE UNIVERSIT"AT DORTMUND}\\
%\hspace*{-1.2cm} \rule{5mm}{5mm} \hspace*{0.1cm} FACHBEREICH INFORMATIK\\
\end{minipage}

\vspace*{4cm}

\hspace*{\links}
\hspace*{-0.2cm}
\begin{minipage}{9cm}
\large
\begin{center}
{\Large Masterarbeit} \\
\vspace*{1cm}
\textbf{Active Automata Learning with Adaptive Distinguishing Sequences} \\
\vspace*{1cm}
Markus Theo Frohme\\
% \vspace*{1cm}
%\today
21. September, 2015
\end{center}
\end{minipage}
\normalsize
\vspace*{5.5cm}

% \hspace*{\links}

\vspace*{2.1cm}

\hspace*{\links}
\begin{minipage}[b]{5cm}
% \normalsize
\raggedright
Gutachter: \\
Prof. Dr. Bernhard Steffen \\
Dipl.-Inf. Malte Isberner \\
\end{minipage}

\vspace*{2.5cm}
\hspace*{\links}
\begin{minipage}[b]{8cm}
% \normalsize
\raggedright
Technische Universität Dortmund \\
Fakultät für Informatik\\
Lehrstuhl für Programmiersysteme\\
\url{http://ls5-www.cs.tu-dortmund.de}
\end{minipage}

\end{titlepage}

